Smoothed Analysis of the Koml\'os Conjecture

The well-known Koml\'os conjecture states that given $n$ vectors in $\mathbb{R}^d$ with Euclidean norm at most one, there always exists a $\pm 1$ coloring such that the $\ell_{\infty}$ norm of the signed-sum vector is a constant independent of $n$ and $d$. We prove this conjecture in a smoothed analysis setting where the vectors are perturbed by adding a small Gaussian noise and when the number of vectors $n =\omega(d\log d)$. The dependence of $n$ on $d$ is the best possible even in a completely random setting. Our proof relies on a weighted second moment method, where instead of considering uniformly randomly colorings we apply the second moment method on an implicit distribution on colorings obtained by applying the Gram-Schmidt walk algorithm to a suitable set of vectors. The main technical idea is to use various properties of these colorings, including subgaussianity, to control the second moment.

==> preamble.tex <==
\newcommand{\wF}{\mathsf{wF}}
\newcommand{\ip}[2]{\langle #1, #2 \rangle}
\newcommand{\supp}{\mathsf{supp}}
%\def\proofname{proof}
%
\newcommand{\IGNORE}[1]{}
%\newcounter{note}[section]
%\newcommand{\haotian}[1]{\refstepcounter{note}$\ll${\bf Haotian~\thenote:} {\sf \color{blue}  #1}$\gg$\marginpar{\tiny\bf HJ~\thenote}}
\newcommand{\haotian}[1]{{\color{red} \textbf{Haotian:} #1}}
\newcommand{\sahil}[1]{{\color{blue} \textbf{Sahil:} #1}}

\newcommand{\nikhil}[1]{{\color{blue} \textbf{Nikhil:} #1}}

\newcommand{\makrand}[1]{{\color{teal} \textbf{Makrand:} #1}}

\newcommand{\bm}{\mathbf}
\newcommand{\price}{\pi}
\newcommand{\probed}{\mathsf{Probed}}
\newcommand{\val}{\mathsf{val}}
\newcommand{\cost}{\mathsf{cost}}
\newcommand{\len}{\mathsf{length}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\setR}{\mathbb{R}}
\newcommand{\setC}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}_{\geq 0}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\A}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\B}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\p}{\ensuremath{\mathbb{P}}}
\newcommand{\Fi}{\ensuremath{\F_{-i}}}
\newcommand{\oi}{\ensuremath{\hat{o}_i}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\T}{\mathcal{T}}
\renewcommand{\S}{\ensuremath{\mathcal{S}}\xspace}

\newcommand{\frugal}{\text{\sc{Frugal}}\xspace}
\newcommand{\POI}{PoI\xspace}
\newcommand{\FreeInfo}{Free-Info\xspace}
\newcommand{\taumax}{\tau^{\max}}
\newcommand{\taumin}{\tau^{\min}}
\newcommand{\Ym}{\Y_{M}}
\newcommand{\Ymax}{Y^{\max}}
\newcommand{\bYmax}{\mathbf{Y^{\max}}}
\newcommand{\Ymmax}{\Ym^{\max}}
\newcommand{\bYmin}{\mathbf{Y^{\min}}}
\newcommand{\Ymin}{Y^{\min}}
\newcommand{\Clients}{\text{\sc{Clients}}}
\newcommand{\leaf}{l}
\newcommand{\one}{\textsf{1}\xspace}
\newcommand{\dd}{\ensuremath{\mathrm{d}}}
\newcommand{\ind}{\ensuremath{\mathbf{1}}}
\newcommand{\eat}[1]{}
\newcommand{\hide}[1]{{\Large \color{red} Contents here are hidden! To reveal contents, remove this command.}}

\newcommand{\OPT}{\ensuremath{\textsf{OPT}} \xspace}
\newcommand{\ALG}{\textsf{ALG}\xspace}

\newcommand{\dum}{\ensuremath{\mathrm{dum}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\trajProf}{\ensuremath{\mathbf{\mathcal{\omega}}}}
\newcommand{\envy}{\ensuremath{\mathsf{envy}}\xspace}
\newcommand{\parent}{\ensuremath{\mathsf{par}}\xspace}
\newcommand{\ancestor}{\ensuremath{\mathsf{Anc}}}
\newcommand{\child}{\ensuremath{\mathsf{Child}}}
\newcommand{\disc}{\ensuremath{\mathrm{disc}}}
\newcommand{\bal}{\ensuremath{\mathsf{bal}}}
\newcommand{\polylog}{\ensuremath{\mathrm{polylog}}\xspace}
\newcommand{\poly}{\ensuremath{\mathrm{poly}}}
\newcommand{\arr}{\ensuremath{\textrm{arr}}}
\newcommand{\col}{\ensuremath{\chi}}
\newcommand{\pref}{P}
\newcommand{\glob}{G}
\newcommand{\CE}{\mathcal{E}}
\newcommand{\CG}{\mathcal{G}}
\newcommand{\loc}{{\textrm{loc}}}
\newcommand{\assign}{\textsf{ind}}
\newcommand{\token}{\textsf{Token}}
\newcommand{\dang}{\mathsf{dangerous}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\valuation}{\mathbf{v}}
\renewcommand{\Re}{\mathrn{Re}}
\newcommand{\tr}{\mathsf{tr}}
\newcommand{\diag}{\mathrm{diag}}

\newcommand{\Def}{\textrm{def}}
\newcommand{\op}{\ensuremath{\mathrm{op}}\xspace}
\global\long\def\norm#1{\left\Vert #1\right\Vert }

\newcommand{\sv}{\mathsf{sv}}
\renewcommand{\ss}{\mathsf{ss}}
%\newcommand{\st}{\mathsf{st}}
\newcommand{\sr}{\mathsf{sr}}

\newcommand{\spn}{\mathsf{span}}
\newcommand{\pdisc}{\mathsf{pdisc}}
\newcommand{\hpdisc}{\mathsf{herpdisc}}
\newcommand{\herdisc}{\mathsf{herdisc}}
\newcommand{\detlb}{\mathsf{detLB}}
\newcommand{\vol}{\mathsf{vol}}
\newcommand{\vlb}{\mathsf{volLB}}
\newcommand{\pvdisc}{\mathsf{pvdisc}}
\newcommand{\hpvdisc}{\mathsf{herpvdisc}}
\newcommand{\vecdisc}{\mathsf{vecdisc}}
\newcommand{\hvdisc}{\mathsf{hervdisc}}
\newcommand{\cdisc}{\mathsf{cdisc}}
\newcommand{\hercdisc}{\mathsf{hercdisc}}
\newcommand{\SDP}{\mathsf{SDP}}
\newcommand{\conv}{\mathsf{conv}}
\newcommand{\diam}{\mathsf{diam}}
\newcommand{\CU}{\mathcal U}
\newcommand{\CN}{\mathcal N}
\renewcommand{\Pr}{\p}
\newcommand{\pmone}{\{\pm 1\}}

